Inferring Rewards from Language in Context

In classic instruction following, language like "I'd like the JetBlue flight" maps to actions (e.g., selecting that flight). However, language also conveys information about a user's underlying reward function (e.g., a general preference for JetBlue), which can allow a model to carry out desirable actions in new contexts. We present a model that infers rewards from language pragmatically: reasoning about how speakers choose utterances not only to elicit desired actions, but also to reveal information about their preferences. On a new interactive flight-booking task with natural language, our model more accurately infers rewards and predicts optimal actions in unseen environments, in comparison to past work that first maps language to actions (instruction following) and then maps actions to rewards (inverse reinforcement learning).

==> sections/630-oracle-switching.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=.75\linewidth]{figs/63-acc_switching.pdf}
\caption{Comparison between our model and a model that switches between updating the posterior with the action- and belief-only model, given oracle access to their accuracies after updating on each round.}
\label{fig:oracle-switching}
\end{figure}
